Edge-aware baselines for ogbn-proteins in PyTorch Geometric: species-wise normalization, post-hoc calibration, and cost-accuracy trade-offs

We present reproducible, edge-aware baselines for ogbn-proteins in PyTorch Geometric (PyG). We study two system choices that dominate practice: (i) how 8-dimensional edge evidence is aggregated into node inputs, and (ii) how edges are used inside message passing. Our strongest baseline is GraphSAGE with sum-based edge-to-node features. We compare LayerNorm (LN), BatchNorm (BN), and a species-aware Conditional LayerNorm (CLN), and report compute cost (time, VRAM, parameters) together with accuracy (ROC-AUC) and decision quality. In our primary experimental setup (hidden size 512, 3 layers, 3 seeds), sum consistently beats mean and max; BN attains the best AUC, while CLN matches the AUC frontier with better thresholded F1. Finally, post-hoc per-label temperature scaling plus per-label thresholds substantially improves micro-F1 and expected calibration error (ECE) with negligible AUC change, and light label-correlation smoothing yields small additional gains. We release standardized artifacts and scripts used for all of the runs presented in the paper.

==> tables/gin_baselines.tex <==
\begin{table}[H]\centering\small\n\begin{tabular}{lccccccccc}\n\toprule\nModel & Norm & Edge$\to$node & Layers & Hid & Edge scalar & Val AUC & Test AUC & Test F1 & Params\\\n\midrule\ngin & bn & sum & 3 & 512 & sum & 0.845 ± 0.002 & 0.761 ± 0.006 & 0.149 ± 0.008 & 0.852 ± 0.000\\\n\bottomrule\n\end{tabular}\n\caption{GIN baselines (enhanced).}\n\label{tab:gin}\n\end{table}\n
